OFDM-based Waveforms for Joint Sensing and Communications Robust to Frequency Selective IQ Imbalance

Orthogonal frequency-division multiplexing (OFDM) is a promising waveform candidate for future joint sensing and communication systems. It is well known that the OFDM waveform is vulnerable to in-phase and quadrature-phase (IQ) imbalance, which increases the noise floor in a range-Doppler map (RDM). A state-of-the-art method for robustifying the OFDM waveform against IQ imbalance avoids an increased noise floor, but it generates additional ghost objects in the RDM [1]. A consequence of these additional ghost objects is a reduction of the maximum unambiguous range. In this work, a novel OFDM-based waveform robust to IQ imbalance is proposed, which neither increases the noise floor nor reduces the maximum unambiguous range. The latter is achieved by shifting the ghost objects in the RDM to different velocities such that their range variations observed over several consecutive RDMs do not correspond to the observed velocity. This allows tracking algorithms to identify them as ghost objects and eliminate them for the follow-up processing steps. Moreover, we propose complete communication systems for both the proposed waveform as well as for the state-of-the-art waveform, including methods for channel estimation, synchronization, and data estimation that are specifically designed to deal with frequency selective IQ imbalance which occurs in wideband systems. The effectiveness of these communication systems is demonstrated by means of bit error ratio (BER) simulations.

==> SA_Radar_Measurements.tex <==


\section{Radar Measurement Results} \label{sec:SA_Radar_Measurements}

This section presents the measurement results as well as an \ac{snr} comparison. 

The system parameters include a carrier frequency $f_\text{c} = 76.6\, \text{GHz}$, with a bandwidth $B = 1\, \text{GHz}$, $N_\text{c} = 1024$ subcarriers and $N_\text{sym} = 256$ \ac{ofdm} symbols. The length of the \ac{cp} is $T_\text{cp} = 1\, \mu\text{s}$. The measurements were conducted in a semi-anechoic chamber with two static \acp{cr} located at distances of $1.3\, \text{m}$ and  $4.1\, \text{m}$. The radar cross section of each of the \acp{cr} is $10\, \text{dBsm}$ and both TX and RX are equipped with standard gain horn antennas each with a gain of $20\, \text{dBi}$. The \ac{bb} \ac{ofdm} signal is generated by an arbitrary waveform generator (Keysight M8195A) and up-converted to $f_\text{c}$ by a Radiometer Physics ZRX90 module. The receiver consists of two \acp{lna} with a total gain of $40\, \text{dB}$ and a noise figure of approx. $3\, \text{dB}$. The relatively high \ac{lna} gain is required to compensate the up- and down-conversion losses to and from $f_\text{c}$. Down-conversion of the \ac{rf}-RX signal is realized in a spectrum analyzer (Rohde \& Schwarz FSW85) and the \ac{bb}-RX signal is digitized by a digital oscilloscope (Keysight DSO91204A). All components are synchronized by a 10-MHz reference signal.

The obtained range profiles are shown in Fig.~\ref{fig:Radar_Measurements} for a standard \ac{ofdm} radar system, an \ac{sa}-\ac{ofdm} radar system with $\kappa=2$, and an \ac{sa}-\ac{ofdm} radar system with $\kappa=4$. For the latter two, we obtained $N_\text{A}=342$ and $N_\text{A}=205$, respectively. 

Estimation of the noise floor is achieved by evaluating the median value of the range profile in a linear scale. The \ac{snr} values are then given by the difference between the highest peak in the range profile and the noise floor. The \ac{snr} values obtained this way are $35.7\, \text{dB}$ for the standard \ac{ofdm} radar system, $32.6\, \text{dB}$ for the \ac{sa}-\ac{ofdm} radar system with $\kappa=2$, and $30.7\, \text{dB}$ for the \ac{sa}-\ac{ofdm} radar system with $\kappa=4$. The loss in \ac{snr} performance compared to the standard \ac{ofdm} radar system is in accordance with the theoretical analysis carried out in Sec.~\ref{sec:Theoretical_SNR}.


\input{./fig/Fig_Radar_Measurements}


